Benchmarking Instance-Centric Counterfactual Algorithms for XAI: From White Box to Black Box

This study investigates the impact of machine learning models on the generation of counterfactual explanations by conducting a benchmark evaluation over three different types of models: a decision tree (fully transparent, interpretable, white-box model), a random forest (semi-interpretable, grey-box model), and a neural network (fully opaque, black-box model). We tested the counterfactual generation process using four algorithms (DiCE, WatcherCF, prototype, and GrowingSpheresCF) in the literature in 25 different datasets. Our findings indicate that: (1) Different machine learning models have little impact on the generation of counterfactual explanations; (2) Counterfactual algorithms based uniquely on proximity loss functions are not actionable and will not provide meaningful explanations; (3) One cannot have meaningful evaluation results without guaranteeing plausibility in the counterfactual generation. Algorithms that do not consider plausibility in their internal mechanisms will lead to biased and unreliable conclusions if evaluated with the current state-of-the-art metrics; (4) A counterfactual inspection analysis is strongly recommended to ensure a robust examination of counterfactual explanations and the potential identification of biases.

==> acm-table_num_data.tex <==

\begin{table}[!h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|l|cccc|ccccc|cccc|}
\hline
&   &       
& \multicolumn{4}{c?}{{\textbf{Proximity}}} 
& \multicolumn{5}{c?}{{\textbf{Interpretability}}}  
& \multicolumn{4}{c|}{{\textbf{Functionality}}} \\
\cline{4-16} 
\multirow{-2}{*}{\textbf{Dataset}}                
& \multirow{-2}{*}{{\textbf{ML Model}}}             
& \multirow{-2}{*}{\textbf{Counterfactual}} 
& \multicolumn{1}{c|}{\textbf{L$_1$-norm}}   
& \multicolumn{1}{c|}{\textbf{L$_2$-norm}}   
& \multicolumn{1}{c|}{\textbf{IMAD}}  
& \multicolumn{1}{c?}{\textbf{MD}}   
& \multicolumn{1}{c|}{\textbf{Spa}}
& \multicolumn{1}{c|}{\textbf{SpaRate}}
& \multicolumn{1}{c|}{\textbf{Pla}}
& \multicolumn{1}{c|}{\textbf{Fea}}
& \multicolumn{1}{c?}{\textbf{Div}} 
& \multicolumn{1}{c|}{\textbf{Com}} 
& \multicolumn{1}{c|}{\textbf{Sta}}
& \multicolumn{1}{c|}{\textbf{Cov}}  
& {\textbf{Eff}}   \\ \hline



% %%% BREAST CANCER
% %%% DECISION TREE
% %%% DICE
 &  & {\textbf{DiCE}}\whitecheck
 & \multicolumn{1}{c|}{{0.94}}              % L1 
 & \multicolumn{1}{c|}{{0.68}}              % L2
 & \multicolumn{1}{c|}{{0.37}}              % IMAD-L1
 & \multicolumn{1}{c?}{0.10}                % MD
 & \multicolumn{1}{c|}{2.43}                % Spa
 & \multicolumn{1}{c|}{0.08}                % SpaRate
 & \multicolumn{1}{c|}{{\greencheck}}       % Pla
 & \multicolumn{1}{c|}{{\\greencheck}}       % Fea
 & \multicolumn{1}{c?}{\greencheck}         % Div
 & \multicolumn{1}{c|}{{\greencheck}}       % Com
 & \multicolumn{1}{c|}{{\crosscheck}}       % Sta
 & \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}} % Cov
 & {0.03}  \\                               % Eff
 \cline{3-16} 
 
% %%% DECISION TREE
% %%% UNJUSTIFIED
&   & \textbf{GrowingSpheresCF}\whitecheck                       
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.13*}}} % L1       
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.11*}}} % L2   
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.04*}}} % IMAD-L1  
& \multicolumn{1}{c?}{\cellcolor{myBlue} \textbf{0.02*}}  % MD
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.73*}}}  % Spa   
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.06*}}} % SpaRate 
& \multicolumn{1}{c|}{\crosscheck}                        % Pla
& \multicolumn{1}{c|}{\crosscheck}                        % Fea
& \multicolumn{1}{c?}\crosscheck                          % Div
& \multicolumn{1}{c|}{\crosscheck}                        % Com
& \multicolumn{1}{c|}{\crosscheck}                        % Sta 
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}} % Cov
& 0.13  \\                                                % Eff
\cline{3-16} 

% %%% DECISION TREE
% %%% PROTOTYPE
&   & \textbf{Prototype}\whitecheck                  
& \multicolumn{1}{c|}{9.83}                 % L1    
& \multicolumn{1}{c|}{2.06}                 % L2  
& \multicolumn{1}{c|}{2.98}                 % IMAD-L1       
& \multicolumn{1}{c?}{1.05}                 % MD
& \multicolumn{1}{c|}{29.60}                % Spa         
& \multicolumn{1}{c|}{0.99}                 % SpaRate          
& \multicolumn{1}{c|}{\crosscheck}          % Pla        
& \multicolumn{1}{c|}{\crosscheck}          % Fea   
& \multicolumn{1}{c?}\crosscheck            % Div
& \multicolumn{1}{c|}{\greencheck}          % Com        
& \multicolumn{1}{c|}{\greencheck}          % Sta 
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{0.25}}} % Cov 
& 24.72  \\ \cline{3-16}                    % Eff

% %%% DECISION TREE
% %%% WATCHER
& \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Decision} \\ \textbf{Tree}\end{tabular}}  
& {\textbf{WatcherCF}\whitecheck}                    
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{24.84}}} % L1
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{4.58}}}  % L2
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{8.90}}}  % IMAD-L1 
& \multicolumn{1}{c?}{\cellcolor{myOrange}{\textbf{2.26}}}  % MD
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{30.00}}} % Spa
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{1.00}}}  % SpaRate
& \multicolumn{1}{c|}{{\crosscheck}}        % Pla
& \multicolumn{1}{c|}{{\crosscheck}}        % Fea
& \multicolumn{1}{c?}{\crosscheck}          % Div
& \multicolumn{1}{c|}{{\crosscheck}}        % Com
& \multicolumn{1}{c|}{{\greencheck}}        % Sta
& \multicolumn{1}{c|}{{0.75}}               % Cov
& {2.05}  \\ \cline{2-16}                   % Eff

% %%% RANDOM FOREST
% %%% DICE
&  
& {\textbf{DiCE}}\whitecheck               %                       
& \multicolumn{1}{c|}{{3.13}}               % L1
& \multicolumn{1}{c|}{{1.29}}               % L2 
& \multicolumn{1}{c|}{{1.01}}               % IMAD-L1 
& \multicolumn{1}{c?}{0.34}                 % MD
& \multicolumn{1}{c|}{{7.40}}               % Spa
& \multicolumn{1}{c|}{{0.25}}               % SpaRate
& \multicolumn{1}{c|}{{\greencheck}}        % Pla
& \multicolumn{1}{c|}{{\greencheck}}        % Fea
& \multicolumn{1}{c?}{\greencheck}                             % Div
& \multicolumn{1}{c|}{{\greencheck}}        % Com
& \multicolumn{1}{c|}{{\crosscheck}}        % Sta
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}}  % Cov
& {0.13}  \\ \cline{3-16}                   % Eff


&                                                   
& {\textbf{GrowingSpheresCF}}\whitecheck                           
& \multicolumn{1}{c|}{{0.73}}               % L1
& \multicolumn{1}{c|}{{0.29}}               % L2
& \multicolumn{1}{c|}{{0.24}}               % IMAD-L1 
& \multicolumn{1}{c?}{0.08}                 % MD
& \multicolumn{1}{c|}{{7.36}}               % Spa
& \multicolumn{1}{c|}{0.25}                 % SpaRate
& \multicolumn{1}{c|}{{\crosscheck}}        % Pla
& \multicolumn{1}{c|}{{\crosscheck}}        % Fea
& \multicolumn{1}{c?}{\crosscheck}          % Div
& \multicolumn{1}{c|}{{\crosscheck}}        % Com
& \multicolumn{1}{c|}{{\crosscheck}}        % Sta
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}}     % Cov
& {0.63}  \\ \cline{3-16}                   % Eff

&                                                   
& \textbf{Prototype}\whitecheck                               
& \multicolumn{1}{c|}{9.83}                 % L1               
& \multicolumn{1}{c|}{2.06}                 % L2       
& \multicolumn{1}{c|}{2.98}                 % IMAD-L1  
& \multicolumn{1}{c?}{1.05}                 % MD 
& \multicolumn{1}{c|}{29.60}                % Spa     
& \multicolumn{1}{c|}{0.99}                 % SpaRate      
& \multicolumn{1}{c|}{\crosscheck}          % Pla
& \multicolumn{1}{c|}{\crosscheck}          % Fea   
& \multicolumn{1}{c?}\crosscheck            % Div
& \multicolumn{1}{c|}{\greencheck}          % Com        
& \multicolumn{1}{c|}{\greencheck}          % Sta 
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{0.25}}} % Cov
& {\cellcolor{myOrange}{\textbf{254.70}}} \\ \cline{3-16}  % Eff
            
            
& \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Random} \\ \textbf{Forest}\end{tabular}}  
& \textbf{WatcherCF}\whitecheck 
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{24.84}}} % L1          
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{4.58}}}  % L2   
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{8.90}}}  % IMAD-L1        
& \multicolumn{1}{c?}{\cellcolor{myOrange}{\textbf{2.26}}}  % MD
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{30.00}}} % Spa        
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{1.00}}}  % SpaRate        
& \multicolumn{1}{c|}{\crosscheck}          % Pla     
& \multicolumn{1}{c|}{\crosscheck}          % Fea        
& \multicolumn{1}{c?}\crosscheck            % Div
& \multicolumn{1}{c|}{\crosscheck}          % Com        
& \multicolumn{1}{c|}{\greencheck}          % Sta   
& \multicolumn{1}{c|}{0.75}                 % Cov  
& 63.71 \\ \cline{2-16}                     % Eff


&   
& {\textbf{DiCE}}\whitecheck   
& \multicolumn{1}{c|}{{1.35}}                                   % L1
& \multicolumn{1}{c|}{{0.93}}                                   % L2
& \multicolumn{1}{c|}{{0.48}}                                   % IMAD-L1
& \multicolumn{1}{c?}{0.16}                                     % MD
& \multicolumn{1}{c|}{{2.46}}                                   % Spa
& \multicolumn{1}{c|}{{0.08}}                                   % SpaRate
& \multicolumn{1}{c|}{{\greencheck}}                            % Pla
& \multicolumn{1}{c|}{{\greencheck}}                            % Fea
& \multicolumn{1}{c?}{\greencheck}                              % Div
& \multicolumn{1}{c|}{{\greencheck}}                            % Com
& \multicolumn{1}{c|}{{\crosscheck}}                            % Sta
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}}       % Cov
& {\cellcolor{myBlue}{\textbf{0.01*}}} \\                       % Eff
\cline{3-16}                  


&   
& \textbf{GrowingSpheresCF}\whitecheck
& \multicolumn{1}{c|}{1.04}                 % L1         
& \multicolumn{1}{c|}{0.33}                 % L2   
& \multicolumn{1}{c|}{0.38}                 % IMAD-L1   
& \multicolumn{1}{c?}{0.08}                 % MD
& \multicolumn{1}{c|}{12.06}                % Spa    
& \multicolumn{1}{c|}{0.40}                 % SpaRate
& \multicolumn{1}{c|}{\crosscheck}          % Pla
& \multicolumn{1}{c|}{\crosscheck}          % Fea    
& \multicolumn{1}{c?}\crosscheck            % Div
& \multicolumn{1}{c|}{\crosscheck}          % Com   
& \multicolumn{1}{c|}{\crosscheck}          % Sta 
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}}   % Cov
& 4.45  \\ \cline{3-16}                     % Eff


&   
& \textbf{Prototype}\whitecheck                                     
& \multicolumn{1}{c|}{9.83}                 % L1           
& \multicolumn{1}{c|}{2.06}                 % L2   
& \multicolumn{1}{c|}{2.98}                 % IMAD-L1   
& \multicolumn{1}{c?}{1.05}                 % MD
& \multicolumn{1}{c|}{29.60}                % Spa     
& \multicolumn{1}{c|}{0.99}                 % SpaRate      
& \multicolumn{1}{c|}{\crosscheck}          % Pla         
& \multicolumn{1}{c|}{\crosscheck}          % Fea    
& \multicolumn{1}{c?}\crosscheck            % Div
& \multicolumn{1}{c|}{\greencheck}          % Com
& \multicolumn{1}{c|}{\greencheck}          % Sta 
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{0.25}}}   % Cov  
& 81.60      \\ \cline{3-16}                % Eff


\multirow{-12}{*}{{\begin{tabular}[c]{@{}c@{}}\textbf{Breast}\\ \textbf{Cancer}\end{tabular}}} 
& \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Neural} \\ \textbf{Network}\end{tabular}} 
& \textbf{WatcherCF}\whitecheck 
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{24.84}}}     % L1
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{4.58}}}      % L2       
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{8.90}}}      % IMAD-L1  
& \multicolumn{1}{c?}{\cellcolor{myOrange}{\textbf{2.26}}}      % MD
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{30.00}}}     % Spa        
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{1.00}}}      % SpaRate  
& \multicolumn{1}{c|}{\crosscheck}                              % Pla        
& \multicolumn{1}{c|}{\crosscheck}                              % Fea        
& \multicolumn{1}{c?}\crosscheck                                % Div
& \multicolumn{1}{c|}{\crosscheck}                              % Com        
& \multicolumn{1}{c|}{\greencheck}                              % Sta 
& \multicolumn{1}{c|}{0.75}                                     % Cov 
& 16.76     \\                                                  % Eff 
\hline
\hline

% %%%
% %%% DIABETES
 &   & {\textbf{DiCE}}\whitecheck 
 & \multicolumn{1}{c|}{{0.63}}              % L1
 & \multicolumn{1}{c|}{{0.53}}              % L2
 & \multicolumn{1}{c|}{{0.74}}              % IMAD-L1
 & \multicolumn{1}{c?}{0.08}                                   % MD
 & \multicolumn{1}{c|}{1.53}  % Spa
 & \multicolumn{1}{c|}{0.19}  % SpaRate
 & \multicolumn{1}{c|}{{\greencheck}}       % Pla
 & \multicolumn{1}{c|}{{\greencheck}}       % Fea
 & \multicolumn{1}{c?}\greencheck                              % Div
 & \multicolumn{1}{c|}{{\greencheck}}       % Com
 & \multicolumn{1}{c|}{{\crosscheck}}       % Sta
 & \multicolumn{1}{c|}{\cellcolor{myBlue}{{\textbf{1.00*}}}}  % Cov
 & {\cellcolor{myBlue}{\textbf{0.02*}}}  \\ \cline{3-16}  % Eff
 
 
 
&   & {\textbf{GrowingSpheresCF}}\whitecheck     
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.04*}}}   % L1        
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.04*}}}   % L2  
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.05*}}}   % IMAD-L1   
& \multicolumn{1}{c?}{\cellcolor{myBlue}{\textbf{0.01*}}}   % MD
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.25*}}}   % Spa    
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{0.16*}}}   % SpaRate      
& \multicolumn{1}{c|}{\crosscheck}                          % Pla
& \multicolumn{1}{c|}{\crosscheck}                          % Fea   
& \multicolumn{1}{c?}\crosscheck                            % Div
& \multicolumn{1}{c|}{\crosscheck}                          % Com    
& \multicolumn{1}{c|}{\crosscheck}                          % Sta 
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}}  % Cov
& 0.15  \\ \cline{3-16}                                     % Eff


&   & \textbf{Prototype}\whitecheck   
& \multicolumn{1}{c|}{2.51}                 % L1   
& \multicolumn{1}{c|}{1.09}                 % L2   
& \multicolumn{1}{c|}{2.72}                 % IMAD-L1       
& \multicolumn{1}{c?}{0.23}                 % MD
& \multicolumn{1}{c|}{6.58}                 % Spa    
& \multicolumn{1}{c|}{0.82}                 % SpaRate           
& \multicolumn{1}{c|}{\crosscheck}          % Pla         
& \multicolumn{1}{c|}{\crosscheck}          % Fea        
& \multicolumn{1}{c?}\crosscheck            % Div 
& \multicolumn{1}{c|}{\greencheck}          % Com        
& \multicolumn{1}{c|}{\greencheck}          % Sta
& \multicolumn{1}{c|}{0.60}                 % Cov   
& 22.28     \\ \cline{3-16}                 % Eff


& \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Decision} \\ \textbf{Tree}\end{tabular}}  
& {\textbf{WatcherCF}}\whitecheck  
& \multicolumn{1}{c|}{{5.17}}               % L1
& \multicolumn{1}{c|}{{1.96}}               % L2
& \multicolumn{1}{c|}{{5.49}}               % IMAD-L1
& \multicolumn{1}{c?}{ 0.42}                % MD
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{8.00}}}  % Spa
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{1.00}}}  % SpaRate
& \multicolumn{1}{c|}{{\crosscheck}}        % Pla
& \multicolumn{1}{c|}{{\crosscheck}}        % Fea 
& \multicolumn{1}{c?}{\crosscheck}          % Div
& \multicolumn{1}{c|}{{\crosscheck}}        % Com
& \multicolumn{1}{c|}{{\greencheck}}        % Sta
& \multicolumn{1}{c|}{{0.60}}               % Cov
& {1.84}  \\ \cline{2-16}                  % Eff
&           



& {\textbf{DiCE}}\whitecheck                % 
& \multicolumn{1}{c|}{{0.79}}              % L1
& \multicolumn{1}{c|}{{0.60}}              % L2
& \multicolumn{1}{c|}{{0.90}}              % IMAD-L1
& \multicolumn{1}{c?}{ 0.09}                % MD
& \multicolumn{1}{c|}{{1.86}}              % Spa
& \multicolumn{1}{c|}{{0.23}}              % SpaRate
& \multicolumn{1}{c|}{{ \greencheck}}       % Pla
& \multicolumn{1}{c|}{{ \greencheck}}       % Fea
& \multicolumn{1}{c?}{ \greencheck}         % Div
& \multicolumn{1}{c|}{{ \greencheck}}       % Com
& \multicolumn{1}{c|}{{\crosscheck}}        % Sta
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}}   % Cov
& { 0.05}  \\ \cline{3-16}                  % Eff
&     




& {\textbf{GrowingSpheresCF}}\whitecheck
& \multicolumn{1}{c|}{{0.19}}               % L1
& \multicolumn{1}{c|}{{0.10}}               % L2
& \multicolumn{1}{c|}{{0.20}}               % IMAD-L1
& \multicolumn{1}{c?}{0.02}                 % MD
& \multicolumn{1}{c|}{{3.56}}               % Spa
& \multicolumn{1}{c|}{{0.45}}               % SpaRate
& \multicolumn{1}{c|}{{ \crosscheck}}       % Pla
& \multicolumn{1}{c|}{{ \crosscheck}}       % Fea
& \multicolumn{1}{c?}{ \crosscheck}         % Div
& \multicolumn{1}{c|}{{ \crosscheck}}       % Com
& \multicolumn{1}{c|}{{\crosscheck}}        % Sta
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}} % Cov
& { 0.47}  \\ \cline{3-16}                  % Eff
&                            




& \textbf{Prototype}\whitecheck                                 
& \multicolumn{1}{c|}{2.49}                                 % L1  
& \multicolumn{1}{c|}{1.10}                                 % L2   
& \multicolumn{1}{c|}{2.68}                                 % IMAD-L1  
& \multicolumn{1}{c?}{0.23}                                 % MD
& \multicolumn{1}{c|}{6.33}                                 % Spa    
& \multicolumn{1}{c|}{0.79}                                 % SpaRate     
& \multicolumn{1}{c|}{\crosscheck}                          % Pla       
& \multicolumn{1}{c|}{\crosscheck}                          % Fea        
& \multicolumn{1}{c?}\crosscheck                            % Div
& \multicolumn{1}{c|}{\greencheck}                          % Com         
& \multicolumn{1}{c|}{\greencheck}                          % Sta     
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{0.45}}}  % Cov
& {\cellcolor{myOrange}{\textbf{250.11}}} \\                % Eff
\cline{3-16} 




& \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Random} \\ \textbf{Forest}\end{tabular}}  
& \textbf{WatcherCF}\whitecheck  
& \multicolumn{1}{c|}{5.09}                                     % L1
& \multicolumn{1}{c|}{1.95}                                     % L2
& \multicolumn{1}{c|}{5.42}                                     % IMAD-L1
& \multicolumn{1}{c?}{0.41}                                     % MD
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{8.00}}}      % Spa
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{1.00}}}      % SpaRate
& \multicolumn{1}{c|}{\crosscheck}                              % Pla
& \multicolumn{1}{c|}{\crosscheck}                              % Fea
& \multicolumn{1}{c?}\crosscheck                                % Div
& \multicolumn{1}{c|}{\crosscheck}                              % Com
& \multicolumn{1}{c|}{\greencheck}                              % Sta
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{0.45}}}      % Cov
& 54.71 \\                                                      % Eff
\cline{2-16} 


&                                                                            
& {\textbf{DiCE}}\whitecheck                  
& \multicolumn{1}{c|}{{0.73}}                               % L1
& \multicolumn{1}{c|}{{0.61}}                               % L2
& \multicolumn{1}{c|}{{0.84}}                               % IMAD-L1
& \multicolumn{1}{c?}{ 0.09}                                % MD
& \multicolumn{1}{c|}{{1.66}}                               % Spa
& \multicolumn{1}{c|}{{0.21}}                               % SpaRate
& \multicolumn{1}{c|}{{\greencheck}}                        % Pla
& \multicolumn{1}{c|}{{\greencheck}}                        % Fea
& \multicolumn{1}{c?}{ \greencheck}                         % Div
& \multicolumn{1}{c|}{{ \greencheck}}                       % Com
& \multicolumn{1}{c|}{{\crosscheck}}                        % Sta
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}}   % Cov
& { 0.06}  \\                                               % Eff
\cline{3-16} 


&   & {\textbf{GrowingSpheresCF}}\whitecheck                            
& \multicolumn{1}{c|}{{ 0.31}}              % L1
& \multicolumn{1}{c|}{{ 0.15}}              % L2
& \multicolumn{1}{c|}{{ 0.32}}              % IMAD-L1
& \multicolumn{1}{c?}{ 0.03}                % MD
& \multicolumn{1}{c|}{{ 5.17}}              % Spa
& \multicolumn{1}{c|}{{ 0.65}}              % SpaRate
& \multicolumn{1}{c|}{{\crosscheck}}        % Pla
& \multicolumn{1}{c|}{{\crosscheck}}        % Fea
& \multicolumn{1}{c?}{\crosscheck}          % Div
& \multicolumn{1}{c|}{{\crosscheck}}        % Com
& \multicolumn{1}{c|}{{\crosscheck}}        % Sta
& \multicolumn{1}{c|}{\cellcolor{myBlue}{\textbf{1.00*}}} % Cov
& { 2.17}  \\                               % Eff
\cline{3-16} 


&   & {\textbf{Prototype}}\whitecheck                     
& \multicolumn{1}{c|}{{2.60}}              % L1
& \multicolumn{1}{c|}{{1.12}}              % L2
& \multicolumn{1}{c|}{{2.81}}              % IMAD-L1
& \multicolumn{1}{c?}{0.24}                % MD
& \multicolumn{1}{c|}{{6.78}}              % Spa
& \multicolumn{1}{c|}{{0.85}}              % SpaRate
& \multicolumn{1}{c|}{{\crosscheck}}       % Pla
& \multicolumn{1}{c|}{{\crosscheck}}       % Fea
& \multicolumn{1}{c?}{\crosscheck}         % Div
& \multicolumn{1}{c|}{{\greencheck}}       % Com
& \multicolumn{1}{c|}{{\greencheck}}        % Sta
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{0.45}}}  % Cov
& {71.34}\\                               % Eff
\cline{3-16} 


\multirow{-12}{*}{{\textbf{Diabetes}}}  
& \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Neural} \\ \textbf{Network}\end{tabular}} 
& \textbf{WatcherCF}\whitecheck                                         
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{~5.79}}}  % L1   
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{~2.13}}}  % L2 
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{~6.03}}}  % IMAD-L1
& \multicolumn{1}{c?}{\cellcolor{myOrange}{\textbf{~0.47}}}  % MD
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{~8.00}}}  % Spa   
& \multicolumn{1}{c|}{\cellcolor{myOrange}{\textbf{~1.00}}}  % SpaRate  
& \multicolumn{1}{c|}{~\crosscheck}                          % Pla       
& \multicolumn{1}{c|}{~\crosscheck}                          % Fea 
& \multicolumn{1}{c?}{~\crosscheck}                          % Div
& \multicolumn{1}{c|}{~\crosscheck}                          % Com     
& \multicolumn{1}{c|}{~\greencheck}                          % Sta 
& \multicolumn{1}{c|}{~0.55}                                 % Cov
& {14.07} \\                                                 % Eff
\hline





\multirow{12}{*}{ \rotatebox[origin=c]{90}{\textbf{Pima Diabetes}}} &
  \multirow{4}{*}{\textbf{DT}} &
  \textbf{DiCE} &
  \multicolumn{1}{l|}{0.63} &
  \multicolumn{1}{l|}{0.53} &
  \multicolumn{1}{l|}{0.74} &
  0.08 &
  \multicolumn{1}{l|}{1.53} &
  \multicolumn{1}{l|}{0.19} &
    \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\greencheck} &
   \greencheck & 
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{\textbf{1.00}}} &
  \cellcolor{myBlue}{\textbf{0.02}} \\ \cline{3-16} 
 &
   &
  \textbf{GrowingSpheresCF} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{0.04*}} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{0.04*}} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{0.05*}} &
  \cellcolor{myBlue}{0.01*} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{1.25*}} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{0.16*}} &
    \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{1.00*}} &
  0.15 \\ \cline{3-16} 
 &
   &
  \textbf{Prototype} &
  \multicolumn{1}{l|}{2.51} &
  \multicolumn{1}{l|}{1.09} &
  \multicolumn{1}{l|}{2.72} &
  0.23 &
  \multicolumn{1}{l|}{6.58} &
  \multicolumn{1}{l|}{0.82} &
   \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{0.60} &
  22.28 \\ \cline{3-16} 
 &
   &
  \textbf{WachterCF} &
  \multicolumn{1}{l|}{5.17} &
  \multicolumn{1}{l|}{1.96} &
  \multicolumn{1}{l|}{5.49} &
  0.42 &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{8.00}} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{1.00}} &
    \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{0.60} &
  1.84 \\ \cline{2-16} 
 &
  \multirow{4}{*}{\textbf{RF}} &
  \textbf{DiCE} &
  \multicolumn{1}{l|}{0.79} &
  \multicolumn{1}{l|}{0.60} &
  \multicolumn{1}{l|}{0.90} &
  0.09 &
  \multicolumn{1}{l|}{\cellcolor{myBlue}1.86} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.23} &
   \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\greencheck} &
   \greencheck & 
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{1.00}} &
  \cellcolor{myBlue}0.05 \\ \cline{3-16} 
 &
   &
  \textbf{GrowingSpheresCF} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.19} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.10} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.20} &
  \cellcolor{myBlue}0.02 &
  \multicolumn{1}{l|}{3.56} &
  \multicolumn{1}{l|}{0.45} &
    \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{1.00*}} &
  0.47 \\ \cline{3-16} 
 &
   &
  \textbf{Prototype} &
  \multicolumn{1}{l|}{2.49} &
  \multicolumn{1}{l|}{1.10} &
  \multicolumn{1}{l|}{2.68} &
  0.23 &
  \multicolumn{1}{l|}{6.33} &
  \multicolumn{1}{l|}{0.79} &
   \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{0.45}} &
  \cellcolor{myOrange}{250.11} \\ \cline{3-16} 
 &
   &
  \textbf{WachterCF} &
  \multicolumn{1}{l|}{5.09} &
  \multicolumn{1}{l|}{1.95} &
  \multicolumn{1}{l|}{5.42} &
  0.41 &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{8.00}} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{1.00}} &
      \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{0.45}} &
  54.71 \\ \cline{2-16} 
 &
  \multirow{4}{*}{\textbf{NN}} &
  \textbf{DiCE} &
  \multicolumn{1}{l|}{0.73} &
  \multicolumn{1}{l|}{0.61} &
  \multicolumn{1}{l|}{0.84} &
  0.09 &
  \multicolumn{1}{l|}{\cellcolor{myBlue}1.66} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.21} &
    \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\greencheck} &
   \greencheck & 
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{1.00}} &
  \cellcolor{myBlue}0.06 \\ \cline{3-16} 
 &
   &
  \textbf{GrowingSpheresCF} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.31} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.15} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}0.32} &
  \cellcolor{myBlue}0.03 &
  \multicolumn{1}{l|}{5.17} &
  \multicolumn{1}{l|}{0.65} &
    \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\cellcolor{myBlue}{1.00}} &
  2.17 \\ \cline{3-16} 
 &
   &
  \textbf{Prototype} &
  \multicolumn{1}{l|}{2.60} &
  \multicolumn{1}{l|}{1.12} &
  \multicolumn{1}{l|}{2.81} &
  0.24 &
  \multicolumn{1}{l|}{6.78} &
  \multicolumn{1}{l|}{0.85} &
   \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{0.45}} &
  71.34 \\ \cline{3-16} 
 &
   &
  \textbf{WachterCF} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{5.79}} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{2.13}} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{6.03}} &
  \cellcolor{myOrange}{0.47} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{8.00}} &
  \multicolumn{1}{l|}{\cellcolor{myOrange}{1.00}} &
     \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\crosscheck} &
   \crosscheck &
  \multicolumn{1}{l|}{\crosscheck} &
  \multicolumn{1}{l|}{\greencheck} &
  \multicolumn{1}{l|}{0.55} &
  14.07 \\ 
  \hline
  \hline



\end{tabular}
}
\caption{Experimental results for numerical datasets: \textit{IMAD-L$_1$} refers to median absolute deviation; \textit{MD} refers to the Mahalanobis Distance; \textit{Spa} refers to sparsity; \textit{Pla} refer to plausibility; \textit{Fea} refers to feasibility; \textit{Div} refers to diversity; \textit{Cov} refers to coverage; \textit{Com} refers to compatibility; \textit{Sta} refers to stability; and \textit{Eff} refers to efficiency}
\label{tab:num_data}
\end{table}

